One Instruction Does Not Fit All: How Well Do Embeddings Align Personas and Instructions in Low-Resource Indian Languages?

Aligning multilingual assistants with culturally grounded user preferences is essential for serving India's linguistically diverse population of over one billion speakers across multiple scripts. However, existing benchmarks either focus on a single language or conflate retrieval with generation, leaving open the question of whether current embedding models can encode persona-instruction compatibility without relying on response synthesis. We present a unified benchmark spanning 12 Indian languages and four evaluation tasks: monolingual and cross-lingual persona-to-instruction retrieval, reverse retrieval from instruction to persona, and binary compatibility classification. Eight multilingual embedding models are evaluated in a frozen-encoder setting with a thin logistic regression head for classification. E5-Large-Instruct achieves the highest Recall@1 of 27.4\% on monolingual retrieval and 20.7\% on cross-lingual transfer, while BGE-M3 leads reverse retrieval at 32.1\% Recall@1. For classification, LaBSE attains 75.3\% AUROC with strong calibration. These findings offer practical guidance for model selection in Indic multilingual retrieval and establish reproducible baselines for future work\footnote{Code, datasets, and models are publicly available at https://github.com/aryashah2k/PI-Indic-Align.

==> assets/t2_heatmap_bge.tex <==
\begin{table*}[t]
\centering
\tiny
\begin{tabular}{lcccccccccccc}
\toprule
\textbf{Src$\backslash$Tgt} & \textbf{Asm} & \textbf{Ben} & \textbf{Guj} & \textbf{Hin} & \textbf{Kan} & \textbf{Mal} & \textbf{Mar} & \textbf{Ory} & \textbf{Pan} & \textbf{Tam} & \textbf{Tel} & \textbf{Urd} \\
\midrule
\textbf{Asm} & -- & 16.5 & 13.7 & 14.7 & 13.7 & 12.6 & 13.3 & 13.2 & 13.0 & 11.5 & 13.3 & 12.8 \\
\textbf{Ben} & 16.0 & -- & 15.8 & 17.6 & 16.2 & 14.9 & 15.8 & 14.8 & 15.0 & 13.6 & 15.9 & 15.4 \\
\textbf{Guj} & 12.4 & 14.8 & -- & 17.1 & 15.5 & 14.0 & 15.6 & 13.5 & 15.5 & 12.6 & 15.3 & 15.0 \\
\textbf{Hin} & 11.9 & 14.6 & 15.6 & -- & 15.2 & 13.6 & 18.4 & 13.0 & 14.8 & 12.4 & 14.8 & 15.2 \\
\textbf{Kan} & 13.2 & 15.8 & 16.4 & 17.9 & -- & 16.0 & 16.4 & 14.7 & 15.6 & 15.0 & 17.8 & 16.0 \\
\textbf{Mal} & 12.0 & 14.8 & 15.2 & 16.4 & 16.3 & -- & 14.8 & 13.3 & 14.5 & 14.1 & 16.0 & 15.0 \\
\textbf{Mar} & 13.0 & 16.1 & 16.9 & 21.7 & 16.7 & 15.1 & -- & 14.4 & 15.6 & 14.0 & 16.3 & 16.1 \\
\textbf{Ory} & 11.9 & 14.0 & 14.1 & 15.0 & 14.0 & 12.6 & 13.5 & -- & 13.5 & 11.5 & 13.8 & 13.0 \\
\textbf{Pan} & 10.4 & 12.2 & 13.6 & 14.4 & 13.0 & 11.5 & 12.6 & 11.5 & -- & 10.3 & 12.6 & 13.2 \\
\textbf{Tam} & 10.6 & 12.5 & 12.9 & 14.4 & 14.3 & 13.4 & 13.2 & 11.5 & 12.5 & -- & 14.0 & 13.2 \\
\textbf{Tel} & 13.2 & 16.0 & 16.5 & 17.9 & 18.1 & 16.4 & 16.4 & 14.7 & 15.8 & 14.7 & -- & 16.3 \\
\textbf{Urd} & 10.0 & 12.1 & 12.9 & 14.7 & 13.1 & 11.8 & 12.5 & 10.8 & 12.8 & 10.9 & 12.7 & -- \\
\bottomrule
\end{tabular}
\caption{Cross-lingual Recall@1 (\%) heatmap for BGE-M3 on T2. Rows represent source languages (persona), columns represent target languages (instruction). Diagonal entries (monolingual) are omitted.}
\label{tab:t2_heatmap}
\end{table*}


==> assets/t3_heatmap_bge.tex <==
\begin{table*}[t]
\centering
\tiny
\begin{tabular}{lcccccccccccc}
\toprule
\textbf{Src$\backslash$Tgt} & \textbf{Asm} & \textbf{Ben} & \textbf{Guj} & \textbf{Hin} & \textbf{Kan} & \textbf{Mal} & \textbf{Mar} & \textbf{Ory} & \textbf{Pan} & \textbf{Tam} & \textbf{Tel} & \textbf{Urd} \\
\midrule
\textbf{Asm} & -- & 24.7 & 20.3 & 21.9 & 21.1 & 19.9 & 21.1 & 20.4 & 19.1 & 18.1 & 20.9 & 19.2 \\
\textbf{Ben} & 25.3 & -- & 25.0 & 27.3 & 26.4 & 24.5 & 26.2 & 24.2 & 23.4 & 22.3 & 25.9 & 24.1 \\
\textbf{Guj} & 20.3 & 24.5 & -- & 27.3 & 25.9 & 24.0 & 26.5 & 22.9 & 24.2 & 21.0 & 25.1 & 23.5 \\
\textbf{Hin} & 21.7 & 26.2 & 27.1 & -- & 27.4 & 25.2 & 31.1 & 24.1 & 25.5 & 22.6 & 26.4 & 25.9 \\
\textbf{Kan} & 20.3 & 24.4 & 24.8 & 26.6 & -- & 25.2 & 25.9 & 22.8 & 22.8 & 22.6 & 26.7 & 23.2 \\
\textbf{Mal} & 20.0 & 24.3 & 24.2 & 25.8 & 26.3 & -- & 25.0 & 22.2 & 22.4 & 22.9 & 26.0 & 23.6 \\
\textbf{Mar} & 21.1 & 25.1 & 25.9 & 30.9 & 26.4 & 24.5 & -- & 22.9 & 23.7 & 22.1 & 25.7 & 24.1 \\
\textbf{Ory} & 20.5 & 23.8 & 22.8 & 24.5 & 23.8 & 22.1 & 23.5 & -- & 21.7 & 19.8 & 23.1 & 21.0 \\
\textbf{Pan} & 19.3 & 23.0 & 24.4 & 25.9 & 24.1 & 22.4 & 24.2 & 21.8 & -- & 20.0 & 23.4 & 23.0 \\
\textbf{Tam} & 17.6 & 21.3 & 20.9 & 23.0 & 24.0 & 22.6 & 22.2 & 19.4 & 19.7 & -- & 23.4 & 21.1 \\
\textbf{Tel} & 20.5 & 24.9 & 24.8 & 26.6 & 27.5 & 25.6 & 26.1 & 22.8 & 23.3 & 23.1 & -- & 24.1 \\
\textbf{Urd} & 19.7 & 24.1 & 24.1 & 26.5 & 24.9 & 23.8 & 25.0 & 21.6 & 23.7 & 21.8 & 24.7 & -- \\
\bottomrule
\end{tabular}
\caption{Cross-lingual Recall@1 (\%) heatmap for BGE-M3 on T3 (reverse). Rows represent source languages (instruction), columns represent target languages (persona). Compare with T2 heatmap to analyze directionality asymmetries.}
\label{tab:t3_heatmap}
\end{table*}


==> assets/t4_classification.tex <==
\begin{table*}[t]
\centering
\small
\begin{tabular}{lccccc}
\toprule
\textbf{Model} & \textbf{AUROC} & \textbf{AUPRC} & \textbf{Acc} & \textbf{ECE} & \textbf{ECE}$_{\text{cal}}$ \\
\midrule
LaBSE & 75.3 & 62.1 & 72.6 & 0.406 & 0.389 \\
BGE-M3 & 73.5 & 50.9 & 76.8 & 0.512 & 0.514 \\
multilingual-e5-large-instruct & 73.2 & 52.9 & 78.1 & 0.525 & 0.531 \\
DistilUSE-Multi & 71.0 & 66.9 & 66.1 & 0.218 & 0.199 \\
indic-sentence-similarity-sbert & 68.5 & 50.0 & 71.2 & 0.386 & 0.403 \\
indic-sentence-bert-nli & 66.5 & 44.2 & 74.8 & 0.446 & 0.483 \\
Para-XLM-R & 61.6 & 34.7 & 74.2 & 0.489 & 0.484 \\
Para-MPNet & 61.4 & 34.9 & 74.6 & 0.475 & 0.492 \\
\bottomrule
\end{tabular}
\caption{Persona-instruction compatibility classification performance (T4) on test set. Models use frozen embeddings with a thin logistic regression head. AUROC and AUPRC are in \%, Acc is calibrated accuracy (\%). ECE is Expected Calibration Error before and after histogram binning calibration. \textbf{\textit{Takeaway}}: LaBSE leads AUROC (75.3\%) while E5 leads accuracy (78.1\%); models with highest discrimination show worst calibration.}
\label{tab:t4_classification}
\end{table*}

